Do Vision and Language Encoders Represent the World Similarly?

Aligned text-image encoders such as CLIP have become the de facto model for vision-language tasks. Furthermore, modality-specific encoders achieve impressive performances in their respective domains. This raises a central question: does an alignment exist between uni-modal vision and language encoders since they fundamentally represent the same physical world? Analyzing the latent spaces structure of vision and language models on image-caption benchmarks using the Centered Kernel Alignment (CKA), we find that the representation spaces of unaligned and aligned encoders are semantically similar. In the absence of statistical similarity in aligned encoders like CLIP, we show that a possible matching of unaligned encoders exists without any training. We frame this as a seeded graph-matching problem exploiting the semantic similarity between graphs and propose two methods - a Fast Quadratic Assignment Problem optimization, and a novel localized CKA metric-based matching/retrieval. We demonstrate the effectiveness of this on several downstream tasks including cross-lingual, cross-domain caption matching and image classification. Code available at github.com/mayug/0-shot-llm-vision.

==> sec/1_intro.tex <==
\section{Introduction}


The recent success of deep learning on vision-language tasks mainly relies on jointly trained language and image encoders following the success of CLIP and ALIGN \cite{jia2021scaling, radford2021learning}. The standard procedure for training these models aims at aligning text and image representation using a contrastive loss that maximizes the similarity between image-text pairs while pushing negative captions away \cite{gutmann2010noise, oord2018representation, chen2020simple}. This achieves a statistical similarity across the two latent spaces, which is key to retrieving the closest cross-modal representations using cosine similarity. This property is not valid for unaligned encoders, hence, extra transformations are needed to bridge the gap. These transformations can be training a mapping network that captures the prior distribution over the text and image representations \cite{merullo2022linearly}. Authors from \cite{merullo2022linearly} have shown that it is possible to train a linear mapping from the output embeddings of vision encoders to the input embeddings of language models and exhibit impressive performance on image captioning and VQA tasks. This indicates that the representations between the unaligned uni-modal vision and language encoders are sufficiently high level and differ only by a linear transformation. However, this linear layer is trained on a CC-3M consisting of 3 million image caption pairs.

In an ideal scenario, we anticipate an alignment between vision and language encoders as they inherently capture representations of the same physical world. To illustrate this alignment, consider physical world concepts, where a text encoder positions two concepts close to each other based on their textual occurrences. This involves textual descriptions of the concepts and their interactions with the world in the training set, determining their proximity in the text encoder space. The images containing these same two concepts in the physical world would capture scenarios in which these concepts interact with it's environment in the world consequently establishing the closeness of the two concepts in the visual encoder space. For example, the physical world concepts of a beach and surfing could exemplify the alignment between vision and language encoders. Textual descriptions may include descriptions of surfers riding waves along the shoreline or people relaxing on the sandy beach. In the visual encoder, corresponding images would capture the essence of these descriptions, featuring surfboards, waves, and individuals engaged in surfing activities, all set within the beach environment. The close proximity of the "beach" and "surfing" concepts in both encoders would be a result of their inherent association in the physical world, as people typically engage in surfing at beaches. This closeness measure could extend to all concepts in the physical world because of the internet-scale image and text datasets these unimodal encoders are trained on. We thus hypothesize that physical world concepts would exhibit semantically similar graphs in both text and vision encoder spaces, reflecting their representation of the same physical world and their relationships with other objects within it.


% Ideally, we expect an alignment to exist between vision and language encoders since they fundamentally represent the same physical world. For example, consider a toy world of all sets that can be represented as strings of 16 binary values like “0001011110001010”. Further, consider a visualization of this world in images consisting of 4$\times$4 patches, where each pixel can either be on or off, depending on the value of that position in the string. Now, imagine two encoders -- one purely textual and one purely visual that are independently trained on these two representations of the same world. By analogy, we expect a bijective mapping to exist between these two representations obtained from different modalities. 



We then ask the question: If the unaligned image and text encoders are semantically similar, is there a way to connect them in a \textit{0-shot manner?} Do they build a similar representation graph over the same information coming from the two modalities?
We study these questions, revealing key similarities between unaligned image and text encoders, and how these similarities can be exploited for downstream tasks. To this end, we employ Centered Kernel Alignment (CKA) \cite{raghu2021vision, cortes2012algorithms, kornblith2019similarity}, which is known for measuring representation similarity both within and between networks. Thus, we measure the CKA between a variety of unaligned vision and language encoders on the image-caption pairs of the COCO~\cite{mscoco} dataset and show that they have comparable semantic similarities to that of aligned encoders like CLIP. Furthermore, we devise a caption matching downstream task and show using two novel methods that latent space communication between unaligned encoders could be achieved by leveraging the semantic similarities between the cross-modal spaces. Our contributions are:


\begin{itemize}

    \item We present a matching method that seeks to find the permutation of the captions that maximizes the CKA. Hence, We formulate maximizing CKA as a quadratic assignment problem and introduce pre-processing transformations and normalizations that greatly improve the matching performance.

    \item We then propose a novel local CKA metric and use it to perform retrieval between two unaligned embedding spaces, demonstrating compelling performance given that there is no training involved. %competitive with that of CLIP on the COCO caption image retrieval.

    \item COCO to NoCAPS~\cite{agrawal2019nocaps} cross-domain image retrieval as well ImageNet 100~\cite{imagenet} classification tasks despite our method not being optimized to align the representation in any manner demonstrating zero-shot communication between the encoder's latent spaces.

    \item Finally, we show a practical application of our method on cross-lingual caption retrieval by making use of sentence transformers trained in various languages and a CLIP model trained only in English. 
    
\end{itemize}

% We notice that the CKA for a set of image representations and text representations from unaligned encoders are close to 0 when the image, caption pairs are not aligned, so we propose a matching method that seeks to find the permutation of the captions that maximizes the CKA. We formulate maximizing CKA as a quadratic assignment problem and introduce preprocessing transformations and normalizations that greatly improve the matching performance. We then propose a novel local CKA metric and use this to perform retrieval between two unaligned embedding spaces, demonstrating performance competitive with that of CLIP on the MS-COCO caption, image retrieval, MSCOCO to NoCAPS cross-domain caption and image retrieval as well imagenet classification tasks despite our method not being trained to align the representation in any manner demonstrating 0-shot communication between the encoder's latent spaces. Finally, we show a practical application of our method by demonstrating impressive cross-lingual image retrieval performance by making use of sentence transformers trained in various languages and a CLIP model trained only in English. 

% Further, we devise a caption matching downstream task and show using two novel methods that latent space communication between unaligned encoders could be achieved by leveraging the semantic similarities between the cross-modal spaces.



% ? It has been observed that the encoders are only different by an isomorphic transformation. Limber finds




% or defining a relative embedding space dependent on the data itself\cite{moschella2022relative}.

==> sec/summary.tex <==
This paper titled “Do Vision and Language Encoders Represent the World Similarly?” examines whether there is an alignment between vision and language encoders not trained jointly. The study uses Centered Kernel Alignment (CKA) to analyze the latent space structures of vision and language models on image-caption benchmarks and finds striking semantic similar representation spaces between unaligned and aligned encoders (Section 6 and Figure 1). In cases where statistical similarity (as in aligned encoders like CLIP) is absent, the paper demonstrates that matching of unaligned encoders is possible without training a linear layer to map the representations, by exploiting semantic similarities between the spaces.


The paper proposes two methods: a Fast Quadratic Assignment Problem (QAP) optimization (Section 4.1) and a novel localized CKA metric-based matching/retrieval (Section 4.2). These methods are shown to be effective in various downstream tasks such as cross-lingual(Table 4), cross-domain caption matching (Table 2), and image classification (Table 3). The authors present a matching method that maximizes CKA by formulating it as a QAP, introduce transformations and normalizations to improve matching performance and demonstrate the effectiveness of their local CKA metric in retrieval tasks, especially for caption-image retrieval on the COCO dataset and cross-lingual image retrieval.
The research concludes that unaligned image and text encoders, despite not being explicitly trained jointly following the CLIP procedure, have key similarities that can be leveraged for downstream tasks. The paper’s experiments use a range of vision and language encoders and are benchmarked on datasets like COCO, NoCaps, and ImageNet-100.

Finally, the paper showcases a practical application of the method on cross-lingual image retrieval by using sentence transformers trained in various languages and a CLIP vision encoder trained only in English. The study suggests that while encoders like CLIP are explicitly trained for alignment, unaligned encoders exhibit a surprising level of semantic alignment, which can be utilized effectively with the right methodologies.


% \begin{figure*}
%         \centering
%     \includegraphics[width=1\linewidth]{images/0-shot-llm-vlm_method_overview.png}
%     \caption{\textbf{Unaligned Vision and Text Encoders show semantic similarities in their graph structures.} We exploit this semantic similarity to enable 0-shot latent space communication by making use of graph-matching algorithms. }
%     \label{fig:illustrative}
% \end{figure*}
